On the use of the Edgeworth expansion in cosmology I: how to foresee and evade its pitfalls

Non-linear gravitational collapse introduces non-Gaussian statistics into the matter fields of the late Universe. As the large-scale structure is the target of current and future observational campaigns, one would ideally like to have the full probability density function of these non-Gaussian fields. The only viable way we see to achieve this analytically, at least approximately and in the near future, is via the Edgeworth expansion. We hence rederive this expansion for Fourier modes of non-Gaussian fields and then continue by putting it into a wider statistical context than previously done. We show that in its original form, the Edgeworth expansion only works if the non-Gaussian signal is averaged away. This is counterproductive, since we target the parameter-dependent non-Gaussianities as a signal of interest. We hence alter the analysis at the decisive step and now provide a roadmap towards a controlled and unadulterated analysis of non-Gaussianities in structure formation (with the Edgeworth expansion). Our central result is that, although the Edgeworth expansion has pathological properties, these can be predicted and avoided in a careful manner. We also show that, despite the non-Gaussianity coupling all modes, the Edgeworth series may be applied to any desired subset of modes, since this is equivalent (to the level of the approximation) to marginalising over the exlcuded modes. In this first paper of a series, we restrict ourselves to the sampling properties of the Edgeworth expansion, i.e.~how faithfully it reproduces the distribution of non-Gaussian data. A follow-up paper will detail its Bayesian use, when parameters are to be inferred.

==> DivergenceComment.tex <==
We had previously repeatedly mentioned that the Edgeworth series is a divergent series. Given Eq.~(\ref{unig}), this statement can be verified with the usual prerequisites for convergence and divergence. If 
\begin{equation}
 \sum_{n = 1}^\infty c_n
\end{equation}
is a general series, then the conditions for convergence include that the $c_n$ must form a null-series, i.e. the terms of the series approach zero, $c_n \to 0$ for $n \to \infty$. The Edgeworth expansion does not necessarily fulfill this criterion, as its cumulants can increase in general. Further tests for convergence or divergence include the ratio test \lna{Here, people will argue yeeah, but the amplitude of the polyspectra will decrease, blabla.}
\begin{equation}
 \lim_{n \to \infty} \frac{|c_{n+1}|}{|c_n|} = s.
\end{equation}
Provided $s$ exists, for $s < 1$, the series converges absolutely which would then imply the series may be reordered. For $s = 1$, the test is inconclusive, meaning the series may converge or diverge.  Finally, for $s > 1$ the series diverges. The same holds true for the root test
\begin{equation}
 \lim_{n \to \infty} \sqrt[n]{|c_n|} = s.
\end{equation}
To apply these tests to the Edgeworth series, it is handy to rewrite the Hermite tensors as a sum. In fact, we have
\begin{equation}
 H_n(x) = n! \sum_{m = 0}^{\lfloor \frac{n}{2}\rfloor} \frac{(-1)^m}{m! (n-2m)!} \frac{x^{n-2m}}{2^m \kappa_2^{n-m}},
\end{equation}
\lna{where $\lfloor \rfloor$ is the floor function. Employing only the third and the fourth cumulant, the Edgeworth series then follows to be}
\begin{equation}
 \calP(x) = \calG(x,\kappa_2)\left[  \sum_{k = 0}^\infty \sum_{l = 0}^k \sum_{m = 0}^{\lfloor 2k - l/2\rfloor} \frac{(4k -l)!}{l! (k-l)!} \left(\frac{\kappa_3}{3!}\right)^l \left( \frac{\kappa_4}{4!} \right)^{k-l} \frac{(-1)^m x^{4k - l -2m}}{m! (4k - l -2m)! 2^m \kappa_2^{4k-l-m}}  \right].
\end{equation}


We hence arrive at the conclusion that if the Edgeworth expansion for cumulants of cosmological density fields is not carefully cherry-picked to fulfill all requirements necessary for convergence, then no easily-accessible argument will exist that guaranteed convergence. %and it will never converge but we illustrate how to get a faithful prediciton in the following

%convergence is a statement about including infinitely many terms, and actually, this is not of interest to us, since we will anyway just want to include a few terms. Our question is rather, whether including a given term improves or worsens the approximation. If we knew the approximation would converge, then including a term would automatically improve matters, but if it diverges this may not be so. Hence asymptotics
